BrainJanus: A Unified Model for Understanding and Generation across Brain, Vision, and Language

Modeling the bidirectional correspondence between external sensory stimuli and internal neural activity has emerged as a critical frontier in neuroscience. However, existing approaches predominantly treat brain encoding and decoding as isolated tasks, relying heavily on unimodal alignment and external priors while overlooking the brain's intrinsic nature as a multimodal integration system. To address these limitations, we propose BrainJanus, the first unified brain model that integrates brain, vision, and language within a single framework. Specifically, we introduce a Unified Brain Tokenizer to quantize continuous neural dynamics into discrete tokens aligned with visual and linguistic representations in a shared Omni space. Building on this, we utilize an All-in-One autoregressive architecture that leverages next-token prediction to enable seamless any-to-any generation, which encompasses image-to-brain and text-to-brain encoding, and brain-to-image and brain-to-text decoding. Extensive experiments demonstrate that BrainJanus achieves superior performance across diverse benchmarks. Furthermore, our framework exhibits zero-shot generalization and preserves interpretable biological topography, highlighting its potential as a general-purpose brain modeling paradigm. The code is available at \href{https://github.com/HaitaoWuTJU/BrainJanus}{GitHub}.

==> 1_intro_old.tex <==
\section{Introduction}
% Advances in neuroimaging technologies have progressively revealed the structure, activity, and function of the human brain. However, the semantics encoded in brain signals remain challenging for humans to interpret directly. This challenge has attracted growing research interest, leading to substantial progress in decoding both visual and linguistic information from neural activity.
% \begin{quote}
% ``As long as our brain is a mystery, the universe, the reflection of the structure of the brain, will also be a mystery.''\\
% \hfill\hspace*{8em} --- Santiago Ramón y Cajal
% \end{quote}
% \begin{quote}
% ``What I cannot create, I do not understand''\\
% \hfill\hspace*{8em} --- Richard Feynman
% \end{quote}
% \begin{quote}
% ``Just as the Rosetta Stone presented the same content in three written forms to decipher hieroglyphs, BrainRosetta decodes unknown brain signals via known images and text.''\\
% \end{quote}

Neuroscience once inspired the rise of deep learning, and now deep learning is in turn advancing our understanding of the brain — a circle of inspiration between neuroscience and artificial intelligence.
%In the late 19th century, the neuron doctrine established the concept of the brain as a network of discrete, interacting units~\cite{ramon1909histologie}. This biological insight later inspired the propose of artificial neural networks, providing a computational framework to model neural information processing~\cite{mcculloch1943logical,rosenblatt1958perceptron}.
%
Over the past decades, fueled by abundant data and innovations in neural-inspired networks, deep learning has achieved remarkable success~\cite{krizhevsky2012imagenet,vaswani2017attention,radford2021learning} in understanding visual and textual modalities.
%
In return, the advances in deep learning models and brain imaging techniques have sparked the progress in brain decoding tasks, which aim at decoding human perceptual experiences from neural activity in various modalities, such as images (brain-visual decoding)~\cite{shen2019deep,takagi2023high} and language (brain-text decoding)~\cite{anumanchipalli2019speech,tang2023semantic}.
% decoding neural signals into various forms such as image and text.
%Inspired by these advances, brain decoding, the task of interpreting visual perceptual experiences from neural activity, has gained significant momentum. 
%Inspired by these advances, brain decoding, the task of reconstructing visual or textual experiences from neural activity, has gained significant momentum. 
%
%Recent studies have leveraged deep and multimodal representations to decode brain signals into images (brain-visual decoding)~\cite{shen2019deep,takagi2023high} and language (brain-text decoding)~\cite{anumanchipalli2019speech,tang2023semantic}
% Just as the decipherment of the Rosetta Stone opened a window into ancient Egyptian civilization, decoding the neural signal promises to open a window into the workings of the human mind.
% Brain decoding, BCI
Specifically, for brain–visual decoding tasks, researchers ~\cite{li2024visual,song2024decoding,wu2025bridging,rajabi2025human} train EEG and MEG encoders and align their representations with corresponding image features from CLIP~\cite{radford2021learning}, achieving cross-modal alignment between neural signals and visual embeddings. 
%
Earlier work~\cite{scotti2024mindeye2,ozcelik2023natural,takagi2023high,wang2024mindbridge} has focused on decoding fMRI activity and then using diffusion-based generative models~\cite{ho2020denoising} to reconstruct the corresponding visual stimuli from those decoded representations.
In brain–text decoding tasks, studies such as ~\cite{li2025brainflora,li2024realmind} first project brain activity into the CLIP text embedding space, and then generate natural language that including the high-level semantic. 
% caption
% In addition, several works have explored decoding speech-evoked brain signals into text~\cite{wang2022open,yang2024mad}.

Although previous works have made notable progress on brain-to-text and brain-to-image decoding using modality-specific architectures, %treating these tasks as separate pipelines constrains their generalization and fails to capture the inherently multimodal nature of brain activity. 
handling these tasks in separate pipelines constrains generalization and more importantly, overlooks the intrinsically multimodal nature~\cite{ghazanfar2006neocortex} of neural activity.
%
In essence, \textbf{brain signals extend beyond a single modality}, as the human brain continuously integrates sensory, conceptual, and linguistic information to form coherent representations of the world.
Even in visual-stimulus-driven datasets such as the Natural Scenes Dataset (NSD)~\cite{allen2022massive}, neural responses encode not only low-level image features but also abstract, higher-level semantics~\cite{chabal2022language}.
For example, when a subject views an image of a cat, the resulting neural activity reflects not only its visual appearance but also its conceptual and linguistic \textbf{associations}, including the word \textit{cat}. Current single-modality decoding methods neglect these multimodal interactions, yielding an incomplete and lossy interpretation of neural activity.
Therefore, to comprehensively decode neural signals, it is essential to achieve \textbf{brain-visual-language modeling} in a unified semantic space, enabling consistent modeling of brain decoding and encoding across various modalities.
% connect them with both visual and linguistic modalities in a unified semantic space.
% by mapping neural representations onto both visual and linguistic semantic spaces, 
% Recent studies have leveraged large-scale pretrained multimodal models, such as CLIP~\cite{radford2021learning}, to align visual representations decoded from neural activity with image features, and have further employed diffusion-based generators~\cite{ho2020denoising} to reconstruct the corresponding visual stimuli.

%These findings underscore the necessity of integrating multiple modalities by mapping neural representations onto both visual and linguistic semantic spaces.
However, unifying the three modalities remains challenging due to significant heterogeneity among them.
Previous studies have primarily focused on learning the mapping between brain signals and the representations of diffusion models and CLIP models, leveraging the generative capabilities of external models. This approach limits the interaction among different modalities and mainly centers on decoding tasks.
In contrast, we adopt a unified framework for both generation and understanding, which fully captures the relationships among the three modalities. This enables our model to go beyond decoding tasks and also encode brain signals.
% Previous studies have relied on diffusion models to generate images and CLIP text features to interface with language models, necessitating separate branches, which are computationally expensive and prone to inter-branch conflicts~\cite{li2024visual}. 
% Moreover, these studies predominantly focus on decoding neural signals while paying limited attention to their encoding, and if the neural responses to stimuli are not properly generated, decoding the corresponding visual or conceptual information from brain signals is inherently limited.
% 核心句，脑信号本身就是mm，之前的方法，，分开，导致了什么，（重要问题）如果只和单模态对齐会导致什么，，，和所以需要实现三模态的紧密对齐，多模态对齐
% 一些reference
% 如何设计三个模态统一是挑战性的，diffusion，clip，必须不同的branch，一个分支会conflict，计算量大，，，，，，，之前的方法
% 三个模态统一 -> 为什么要引入理解一体化框架
% 因此，我们需要生成理解一体化框架的合理性
% 重点
% 方法更详细一点，自回归框架的优势，所以能够原生同时理解和对齐三种模态的能力，low-high recon，high-level，hint
% 图：多任务，哪些任务，brain-visual，-，-，-，-, 功能
% 雷达图
% brian img text 具体的信号，
% 自回归要表示出来
% 右下角token，容易被误解为输出，其实是legend
% 中间的mllm，stage 1 ，stag2，stage3
% 有点空，体现复杂性
% 大模型文本输出框
% text2img, img2text
% 配色
% brainrosetta，logo
% 脑信号 线条
% Previous studies such as ~\cite{du2023decoding,qiu2025mindllm,li2025brainflora,mai2023unibrain} have explored mapping brain, visual, and linguistic modalities into a shared representation space, and decoding outputs across corresponding modality models, using diffusion models for images and language models for text.
% However, these approaches rely on separate generative architectures for different modalities, which result in representational gaps and limit cross-modal semantic alignment. 
% Therefore, unifying brain, vision, and language within a shared token space to enable bidirectional transformations across the three modalities is of great significance for advancing the interpretation and understanding of neural signals.
% Motivated by these insights, we propose \textbf{BrainRosetta}, a unified framework that aligns brain, vision, and language modalities within a shared token space, enabling cross-modal understanding and generation with next token prediction paradigm. 
Our main contributions are summarized as follows:
\begin{enumerate}
    \item We design a unified architecture that maps brain, vision, and language modalities into a shared token space, enabling bidirectional generation across modalities through next-token prediction.
    \item BrainRosetta integrates VQ-VAE encoders and a Unified Multimodal LLM, achieving coherent token-level alignment and eliminating the need for modality-specific generators.
    \item Experiments demonstrate that BrainRosetta achieves state-of-the-art performance in brain-to-text generation, reconstructs visual scenes with high fidelity from brain signals, and generates semantically meaningful brain activity from visual or textual inputs, while exhibiting strong zero-shot cross-task generalization.
\end{enumerate}
% Large language models (LLMs) have rapidly advanced the capacity of AI systems to process and generate natural language, images, and other modalities. Nevertheless, a critical modality remains comparatively underexplored: the human brain. Neural signals such as functional magnetic resonance imaging (fMRI) are inherently omni-modal, providing a direct yet intricate window into core brain functions that span perception (e.g., vision, audition) and cognition (e.g., reasoning, memory, language).

% Concurrently, unified models for image generation and understanding have recently emerged~\cite{janus,ddd,ddd}, highlighting the potential of bridging multiple modalities within one framework. 

% Motivated by these advances, we introduce NeuroOmni, a unified multimodal large language model (UnifiedMLLM) designed to enable bidirectional transformations across brain, vision, and language modalities. By unifying these domains within a single framework, NeuroOmni paves the way for establishing deeper connections between brain signals and LLMs, which holds the potential to enable transformative applications ranging from brain–computer interfaces to cognitive decoding.

\begin{figure*}[t]
  \centering
    \includegraphics[width=0.96\linewidth]{figs/overview.pdf}
    \caption{An overview of BrainRosetta. The input data, regardless of its modality, is tokenized into a shared token space and then organized into a token sequence. BrainRosetta processes these tokens autoregressively, enabling arbitrary transformations among the brain, image, and text modalities.}
    \label{fig:arch}
\end{figure*}

% To address these challenges, we propose \textbf{NeuroOmni}, a unified framework for multimodal understanding and generation that integrates brain signals into the MLLM ecosystem. At the heart of NeuroOmni is the \textbf{Unify-MLLM (BrainOmni)} model, which learns a shared tokenized representation across brain, image, and text modalities. Modality tokens provide consistent embeddings, while task tokens guide downstream objectives such as decoding text from fMRI or generating images conditioned on neural activity. This design enables bidirectional mappings across all supported modalities, removing the need for task-specific architectures.

% Our contributions are threefold. First, we introduce a general-purpose architecture that seamlessly incorporates brain recordings into the MLLM paradigm. Second, we develop modality-agnostic embedding and de-tokenization layers that enable flexible brain–image–text translation. Third, we demonstrate through experiments that NeuroOmni achieves strong reconstruction of visual and textual content from neural inputs, outperforming baseline models in both accuracy and fidelity. By unifying brain signals with language and vision in a single generative model, NeuroOmni provides a foundation for deeper integration of human cognition with artificial intelligence.


% \textcolor{black}{Through this architecture, \ours{} establishes a unified representation paradigm that facilitates seamless encoding and decoding across brain, vision, and language modalities, as illustrated in~\cref{fig:motivation}. This design yields two distinct advantages: 
% first, it enables flexible brain encoding decoding， 4 tasks in one single model, generation within a single model via autoregressive modeling; 
% second, Zero-shot Cross-task Generalization, only on the fMRI-to-text generation task can also transfer to fMRI-to-image generation.
% 扩充一下
% }
 % third, the unified training strategy enables different tasks to mutually reinforce each other, yielding superior performance on individual benchmarks compared to single-task baselines.
%%%%%%%% Contributions
% 相比传统模型，这种自回归式的多模态brain foundation model有以下几种优点：
% 1.同之前“脑–图像”“脑–语言”两两对齐范式相比，brain-visual-linguisitic三模态对齐的自回归框架可以实现任意两个模态之间的转变，同时实现编码与解码任务，不仅可以生成也可以理解，实现了XX个任务
% 2.我们的方法在xx任务上远超sota，在xx任务上，与diffusion模型取得有竞争力的结果
% 3.能够实现zero-shot任务泛化XXXX，一体化训练可以让模型在不同任务之间共享知识，所以能泛化
% 4.神经活动表明我们的方法所synthetic fMRI signals保留了 interpretable cortical patterns 以及underlying biological neural variability. 
% \textcolor{black}{Our main contributions are summarized as follows:
% \begin{enumerate}
% \item We introduce \ours{}, which, to the best of our knowledge, is the first unified autoregressive model that bridges brain, vision, and language modalities. Unlike prior disjoint pipelines, our framework establishes a shared discrete token space to enable seamless any-to-any generation, unifying encoding and decoding tasks within a single model.
% \item \ours{} delivers competitive performance across diverse encoding and decoding benchmarks. Crucially, our experiments reveal that joint training across tasks yields superior accuracy compared to task-specific models.
% \item By integrating diverse tasks into a unified training paradigm, our model facilitates effective cross-modal knowledge transfer. This synergy enables strong zero-shot generalization to unseen tasks, demonstrating the model's capacity to learn robust, task-agnostic semantic representations.
% \item Beyond empirical metrics, we validate that the synthetic fMRI signals generated by our model preserve interpretable cortical topography and intrinsic biological variability, suggesting that \ours{} captures the underlying neural mechanisms of sensory processing.
% \end{enumerate}
% }

%(2) \textbf{Disjointed representation learning across tasks.} 
% Although encoding (stimuli-to-brain) and decoding (brain-to-stimuli) 
%This disjointed approach yields task-specific representations and 
%, leveraging these features to reconstruct images and captions by projecting them into diffusion and language models, respectively. 

% fundamentally model reciprocal directions of the same neural-visual correspondence, existing paradigms treat them as isolated tasks with separate optimization objectives~\cite{scotti2024mindeye2,wang2024mindbridge}.  
%that fail to mutually enhance one another. 


%However, existing methods fail to account for the fact that brain signals is inherently multimodality, suffer from under-exploited multimodal semantics in brain signals.
%The brain response to a visual scene involves not only low-level visual patterns but also higher-level conceptual and linguistic associations, reflecting a holistic cognitive process. 
%Current methods fail to capture these fine-grained multimodal nuances, [adding supporting evidence].


%%%%% limitation v0126 morning %%%%%%
% However, existing approaches suffer from two fundamental limitations:
% (1) \textbf{Under-exploited multimodal semantics in brain signals.} 
% The human brain is inherently multimodal~\cite{huth2016natural,binder2009semantic}: a visual stimulus elicits not only visual responses but also associated linguistic and semantic concepts. Previous studies~\cite{ralph2017neural} find that semantic representations tile the entire cortex, organizing concepts into domains that are inextricably grounded in sensory modalities such as vision and touch. 
% %
% However, existing methods predominantly rely on uni-modal alignment, restricting themselves to extracting visually-aligned CLIP representations~\cite{scotti2024mindeye2,lin2022mind,xia2024umbrae}, leveraging these features to reconstruct images and captions by projecting them into diffusion and language models, respectively, resulting in suboptimal decoding fidelity. 
%
%(2) \textbf{Disjointed representation learning across tasks.} 
%Although encoding (stimuli-to-brain) and decoding (brain-to-stimuli) fundamentally model reciprocal directions of the same neural-visual correspondence, existing paradigms treat them as isolated tasks with separate optimization objectives~\cite{scotti2024mindeye2,wang2024mindbridge}. This disjointed approach yields task-specific representations that fail to mutually enhance one another. Consequently, this suboptimal learning necessitates an over-reliance on external priors (e.g., Diffusion or LLMs) to supplement the limited semantic content decoded from brain activity.

%%%%%%%%%%%%%%%%%%%%%%%Limitation V1
% However, existing approaches suffer from two fundamental limitations:
% (1)  \textbf{Seperated encoding and decoding modules.} Most existing methods focus exclusively on either encoding~\cite{mai2025synbrain,bao2025mindsimulator} or decoding~\cite{scotti2023reconstructing,zhou2024clip}. While some studies have attempted to achieve bidirectional encoding and decoding, they still rely on two separate networks and optimization objectives for each direction~\cite{wang2024mindbridge, qian2024lea,beliy2019voxels}.
% (2)  \textbf{Separated image and text pipelines.}  Recent studies predominantly focus on extract visually-aligned CLIP representations from brain signals~\cite{scotti2024mindeye2,lin2022mind,xia2024umbrae}, leveraging these features to reconstruct images and captions by projecting them into diffusion and language models, respectively. 
% %
%However, such disjointed approaches fail to account for the fact that brain modality is naturally multimodal. For example, when a human views an image or text description of a cat, the elicited neural activity reflects not only its visual appearance but also higher-level conceptual and linguistic associations.}


==> tabs/ablation_task.tex <==
\begin{table}[t]
\centering
\caption{Ablation study on different training task combinations.}
\label{tab:task_ablation}
\setlength{\tabcolsep}{6pt}
\renewcommand{\arraystretch}{1.15}
\resizebox{\linewidth}{!}{
\begin{tabular}{lcccccccc}
\toprule
\multirow{2}{*}{Training Tasks}
& \multicolumn{2}{c}{Text}
& \multicolumn{2}{c}{Image} \\
\cmidrule(lr){2-3} \cmidrule(lr){4-5}
& BERT~$\uparrow$
& CLIP~$\uparrow$
& Inception~$\uparrow$
& CLIP~$\uparrow$ \\
\midrule
B$\rightarrow$I
& -- & -- & 0.412 & 0.298 \\

B$\rightarrow$T
& 0.623 & 0.351 & -- & -- \\

B$\rightarrow$I + B$\rightarrow$T
& 0.641 & 0.372 & 0.438 & 0.315 \\

B$\rightarrow$I + B$\rightarrow$T + I$\rightarrow$B
& 0.655 & 0.386 & 0.451 & 0.329 \\

Full (All Tasks)
& \textbf{0.671} & \textbf{0.401}
& \textbf{0.468} & \textbf{0.344} \\
\bottomrule
\end{tabular}
}
\end{table}


==> tabs/tmp.tex <==
 % ($\downarrow$)  ($\uparrow$)
% \subsection{Brain-Vision-Language Interactions}

% \begin{table*}[t]
% \centering
% \caption{Quantitative Results for Brain Decoding, Brian Encoding and General Tasks.}
% \resizebox{\linewidth}{!}{
% \begin{tabular}{ccccccccc}
% \toprule
% \textbf{} & \textbf{Task} & \textbf{Metric} & \textbf{UMBRAE} & \textbf{MindBridge} & \textbf{Mindeye2} & \textbf{SynBrain} & \textbf{MindLLM} & \textbf{\ours{}} \\ 
% \midrule

% \multirow{6}{*}{\rotatebox[origin=c]{90}{\textbf{Brain Decoding}}}
% & \multirow{3}{*}{\rotatebox[origin=c]{90}{To Img}} & PixCorr $\uparrow$ &  &  &  &  &  \\ 
% & & SSIM $\uparrow$ &  &  &  &  &  \\ 
% & & Alex(2) $\uparrow$ &  &  &  &  &  \\ 
% % & & Alex(5) $\uparrow$ &  &  &  &  &  \\ 
% % & & Incep $\uparrow$ &  &  &  &  &  \\ 
% % & & CLIP $\uparrow$ &  &  &  &  &  \\ 
% % & & Eff $\downarrow$ &  &  &  &  &  \\ 
% % & & SwAV $\downarrow$ &  &  &  &  &  \\ 
% \cmidrule(lr){2-9}

% & \multirow{3}{*}{\rotatebox[origin=c]{90}{To Text}} 
% & CLIP-T $\uparrow$ & - & - & - & - &0.878 & 0.926 \\ 
% &  & CLIP-I $\uparrow$ & - & - & - & - &0.486 & 0.940 \\ 
% & & BertScore $\uparrow$ &  &  &  &  &0.459 &0.586\\
% & & LLM $\uparrow$ &  &  &  &  &&\\
% \midrule

% \multirow{8}{*}{\rotatebox[origin=c]{90}{\textbf{Brain Encoding}}}
% & \multirow{4}{*}{\rotatebox[origin=c]{90}{From Text}} 
% & MSE $\downarrow$ & - & - & - & - & -\\
% &  & Person $\uparrow$ & - & - & - & - & -\\ 
% &  & Cosine $\uparrow$ & - & - & - & - & -\\ 
% &  & CLIP $\uparrow$ & - & - & - & - & -\\ 
% \cmidrule(lr){2-9}
% & \multirow{4}{*}{\rotatebox[origin=c]{90}{From Brain}}  & MSE $\downarrow$ & - & - & - & - & - \\
% &  & Person $\uparrow$ & - & - & - & - & - \\
% &  & Cosine $\uparrow$ & - & - & - & - & - \\ 
% &  & CLIP $\uparrow$ & - & - & - & - & - \\ 
% \midrule

% \multirow{8}{*}{\rotatebox[origin=c]{90}{\textbf{General Tasks}}}
% & \multirow{4}{*}{\rotatebox[origin=c]{90}{Und.}} & Accuracy & - & - & - & - & - \\
% &  & F1 Score & - & - & - & - & - \\
% &  & F1 Score & - & - & - & - & - \\ 
% &  & F1 Score & - & - & - & - & - \\ 
% \cmidrule(lr){2-9}
% & \multirow{4}{*}{\rotatebox[origin=c]{90}{Gen.}} & Accuracy & - & - & - & - & - \\ 
% &  & F1 Score & - & - & - & - & - \\ 
% &  & F1 Score & - & - & - & - & - \\ 
% &  & F1 Score & - & - & - & - & - \\ 
% \bottomrule
% \end{tabular}
% }
% \end{table*}

% We implement the conversion between Brain-Vision-Language modalities, which includes the following six tasks: reconstruction of visual stimuli from brain signals, text explanation of brain signals, generation of brain signals from visual stimuli, generation of brain signals from text, image-to-text generation, and text-to-image generation. The qualitative and quantitative results are shown in Figure X and Table X, respectively.
% \begin{table*}[t]
% \centering
% \setlength{\tabcolsep}{6pt}
% \renewcommand{\arraystretch}{1.25}
% \caption{Quantitative Results for Brain-Vision-Language Interactions}
% \resizebox{\linewidth}{!}{
% \begin{tabular}{l|ccc|ccccc}
% \toprule
% \multirow{2}{*}{Method} &
% \multicolumn{3}{c|}{Low-Level} &
% \multicolumn{5}{c}{High-Level} \\
% & PixCorr $\uparrow$ & SSIM $\uparrow$ & Alex(2) $\uparrow$
% & Alex(5) $\uparrow$ & Incep $\uparrow$ & CLIP $\uparrow$ & Eff $\downarrow$ & SwAV $\downarrow$ \\
% \midrule
% MindEye2
% & \best{0.322} & \best{0.431} & \best{96.1\%}
% & 98.6\% & \second{95.4\%} & 93.0\% & \best{0.619} & \second{0.344} \\
% MindEye2 (unrefined)
% & 0.278 & 0.328 & \second{95.2\%}
% & \second{99.0\%} & \second{96.4\%} & \second{94.5\%} & \second{0.622} & \second{0.343} \\
% MindEye1
% & \second{0.319} & 0.360 & 92.8\%
% & 96.9\% & 94.6\% & 93.3\% & 0.648 & 0.377 \\
% Ozcelik and VanRullen (2023)
% & 0.273 & \second{0.365} & 94.4\%
% & 96.6\% & 91.3\% & 90.9\% & 0.728 & 0.421 \\
% Takagi and Nishimoto (2023)
% & 0.246 & 0.410 & 78.9\%
% & 85.6\% & 83.8\% & 82.1\% & 0.811 & 0.504 \\
% MindEye2 (low-level)
% & 0.399 & 0.539 & 70.5\%
% & 65.1\% & 52.9\% & 57.2\% & 0.984 & 0.673 \\
% MindEye2 (1 hour)
% & 0.195 & 0.419 & 84.2\%
% & 90.6\% & 81.2\% & 79.2\% & 0.810 & 0.468 \\
% \textbf{\ours{} (Ours)} & 0.195 & 0.419 & 84.2\% & 90.6\% & 81.2\% & 79.2\% & 0.810 & 0.468 \\
% \bottomrule
% \end{tabular}
% }
% \end{table*}
% \begin{table*}[t]
%     \centering
%     % \vspace{-1.7em}
%     \caption{Quantitative Results for Brain Captioning. The metrics for \ours{} except BERTScore\citep{zhang2019bertscore} are reported as obtained from the BrainHub\citep{xia2024umbrae} benchmark for a fair comparison. }
%     \label{tab:caption}
%     \vskip 0.1in
%     \resizebox{\linewidth}{!}{
%     \begin{tabular}{l|ccccccccccc}
%     \toprule
%  % \multirow{2}{*}{Method}&  \multirow{2}{*}{cross-subject}&\multicolumn{5}{c}{fMRI caption} & &  &\\
%    {Method} &{{BLEU-1} $\uparrow$} & {BLEU-2 $\uparrow$} & {BLEU-3 $\uparrow$} & {{BLEU-4} $\uparrow$} &{METEOR $\uparrow$}&{ROUGE $\uparrow$}& {CIDEr $\uparrow$}&{SPICE $\uparrow$}&{CLIP-S $\uparrow$}&{RefCLIP-S $\uparrow$}&{BERTScore $\uparrow$}\\
%     \midrule
%     RealMind & 26.59 & {$-$} & {$-$} & 4.31 & 17.79 & {$-$} & {$-$} & {$-$} & {$-$} & {$-$} & {$-$} \\
%     UMBRAE & 59.44& 40.48& 27.66&19.03&19.45&  43.71& 61.06& 12.79 & 67.78 & 73.54 & {$-$} \\
%     MindLLM & 61.75 & 42.84 & 29.86 & 21.24  &  19.54 & 45.82 & 60.97  & 11.79 & {$-$} & {$-$} & {$-$}\\
%     BrainFLORA(THINGS-EEG2) & 36.36 & 30.80 & 25.76 & 19.67 & 20.01 & 45.86 & 2.86 & 15.62 & 42.74 & 51.80 & {$-$} \\
%     BrainFLORA(THINGS-MEG)  & 36.53 & 31.01 & 25.99 & 19.88 & 19.79 & 46.01 & 3.15 & 15.51 & 43.01 & 51.55 & {$-$}\\
%     BrainFLORA(THINGS-fMRI)   & 37.96 & 31.59 & 26.29 & 20.11 & 20.03 & 46.69 & 4.40 & 15.55 & 44.21 & 52.96 & {$-$}\\
%     \textbf{\ours{} (Ours)}  & {$-$} &  {$-$} & {$-$} & {$-$}  & 
%  {$-$} & {$-$} & {$-$}  & {$-$}  & {$-$}   & {$-$} & {$-$}\\
%     \bottomrule
%     \end{tabular}}
% \end{table*}


% \begin{table}[ht]
%   \centering
%   \resizebox{\linewidth}{!}{
%   \begin{tabular}{lccccccc}
%     \toprule
%     \multirow{2}{*}{Method} 
%       & \multicolumn{2}{c}{Brain Decoding} 
%       & \multicolumn{2}{c}{Brain Encoding} 
%       & \multicolumn{2}{c}{General Tasks} \\
%     \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7}
%       & To Img & To Text & From Img & From Text & Und. & Gen. \\
%     \midrule
%     Brain-Diffuser~\cite{ozcelik2023natural} & \cmark & \xmark & \xmark & \xmark & \xmark & \xmark \\
%     BrainCap~\cite{ozcelik2023natural} & \cmark & \cmark & \xmark & \xmark & \xmark & \xmark \\
%     SDRecon~\cite{takagi2023high} & \cmark & \cmark & \xmark & \xmark & \xmark & \xmark \\
%     MinD-Vis~\cite{chen2023seeing} & \cmark & \xmark & \xmark & \xmark & \xmark & \xmark \\
%     Mind Reader~\cite{lin2022mind} & \cmark & \cmark & \cmark & \xmark & \xmark & \xmark \\
%     UniBrain~\cite{mai2023unibrain} & \cmark & \cmark & \xmark & \xmark & \xmark & \xmark \\
%     MindEye2~\cite{scotti2024mindeye2} & \cmark & \cmark & \xmark & \xmark & \xmark & \xmark \\
%     OneLLM~\cite{han2024onellm} & \xmark & \cmark & \xmark & \xmark & \cmark & \xmark \\
%     UMBRAE~\cite{xia2024umbrae} & \cmark & \cmark & \xmark & \xmark & \xmark & \xmark \\
%     % BrainChat & \cmark & \cmark & \xmark & \xmark & \cmark & \cmark \\
%     MindBridge~\cite{wang2024mindbridge} & \cmark & \xmark & \xmark & \xmark & \xmark & \xmark \\
%     SynBrain~\cite{mai2025synbrain} & \cmark & \xmark & \cmark & \xmark & \xmark & \xmark \\
%     MindLLM~\cite{qiu2025mindllm} & \xmark & \cmark & \xmark & \xmark & \cmark & \xmark \\
%     \ours{} & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark \\
%     \bottomrule
%   \end{tabular}
%   }
%   \caption{Methods and their capabilities in brain decoding/encoding and General Tasks. brain decoding including To img, to text. brain encoding including from brain from text, general including img understading, and Visual Generation}
% \end{table}
